Rethinking Graph Neural Networks for the Graph Coloring Problem

Graph coloring, a classical and critical NP-hard problem, is the problem of assigning connected nodes as different colors as possible. However, we observe that state-of-the-art GNNs are less successful in the graph coloring problem. We analyze the reasons from two perspectives. First, most GNNs fail to generalize the task under homophily to heterophily, i.e., graphs where connected nodes are assigned different colors. Second, GNNs are bounded by the network depth, making them possible to be a local method, which has been demonstrated to be non-optimal in Maximum Independent Set (MIS) problem. In this paper, we focus on the aggregation-combine GNNs (AC-GNNs), a popular class of GNNs. We first define the power of AC-GNNs in the coloring problem as the capability to assign nodes different colors. The definition is different with previous one that is based on the assumption of homophily. We identify node pairs that AC-GNNs fail to discriminate. Furthermore, we show that any AC-GNN is a local coloring method, and any local coloring method is non-optimal by exploring the limits of local methods over sparse random graphs, thereby demonstrating the non-optimality of AC-GNNs due to its local property. We then prove the positive correlation between model depth and its coloring power. Moreover, we discuss the color equivariance of graphs to tackle some practical constraints such as the pre-fixing constraints. Following the discussions above, we summarize a series of rules a series of rules that make a GNN color equivariant and powerful in the coloring problem. Then, we propose a simple AC-GNN variation satisfying these rules. We empirically validate our theoretical findings and demonstrate that our simple model substantially outperforms state-of-the-art heuristic algorithms in both quality and runtime.

==> doc/back.tex <==
\section{Brief Introduction}
This project aims to solve the graph coloring problem, which is NP-hard, by GNN-based method.
Several DL-based methods were proposed to tackle the coloring problem such as \cite{}
\section{Other GNN variations}
GCN
\begin{align}
   \vh_v^{(k)} = \text{ReLU}(\mW\cdot \text{MEAN}\{\vh_u^{(k-1)},\forall u\in N(v) \cup {v} \}),
\end{align}
GIN
\begin{align}
    \vh_v^{(k)} = \text{MLP}^{(k)}(\text{SUM}\{\vh_u^{(k-1)},\forall u\in N(v) \cup {v} \}),
\end{align}
Our Graph Convolution for Coloring
\begin{align}
    \vh_v^{(k)} = \vh_v^{(k-1)} - \alpha \cdot \text{MEAN}\{{\vh_v'^{(k-1)}},\forall u\in N(v) \},
\end{align}

where $\alpha$ is a self-defined step rate, and $\vh_v'^{(k-1)}$ is defined as follows:
\begin{align}
    \vh_v'^{(k-1)} = {\text{softmax}(\vh_v^{(k-1)})} - \frac{1}{|\vh_v^{(k-1)}|}
\end{align}

The intuition is simple: 
The node embedding of each node, i.e., $v$, should be as different from the embedding of corresponding neighbors, i.e., $u\in N(v)$, as possible.

Besides, the node attribute is randomly initialized to make the node embedding of isomorphic nodes different.

\subsection{Results}
\begin{itemize}
    \item Optimal in small cases (number of nodes  $<$ 10). The simplified graphs in ISCAS are all small, therefore it can be solved without additional loss.
    \item Not-optimal in non-simplified cases. The reason is easy to follow. Currently, we only notice two reasons.
\end{itemize}

\subsection{Future Directions}
1. Theory Proof (w. Siu On):
\begin{itemize}
    \item Show that GNNs are at most as powerful as our convolution method in graph coloring problem.
    \item Any Other related work/theory to solve the non-optimality?
\end{itemize}
2. Reason for non-optimality:
\begin{itemize}
    \item Try the general benchmark for graph coloring. 
    \item Study the reason
    \item Maybe we can show that such cases are unsolvable for original GNN-based method
    \item If so, we should solve this by either post-process (not elegant) or by other tricks in GNN.
    \item Otherwise, any Other related work/theory to solve the non-optimality?
\end{itemize}

==> doc/rebuttal.tex <==
We thank the reviewers for their valuable and suggestive comments. 
% We would like to emphasize one of our contributions in the theoretical study about the locality of AC-GNN. 
% In the GNNs community, it is acknowledged that general AC-GNNs are local algorithms since they are constrained by the depth (\# of layers),
% and AC-GNNs can be global (detect the global structure) as long as the network is deep enough.
% %  Similarly, it is believed that an AC-GNN can increase its ability in graph coloring with the increasing of its depth.
% However, in the graph theory community, a local algorithm such as AC-GNNs cannot be global, no matter how deep the network is.
% We provide a formal definition of local/global AC-GNN (Def 3 \& Corollary 2), and further prove that local algorithms are always not optimal in the graph coloring problem (Corollary 1).
% Therefore, to strengthen its power in graph coloring, a global scheme should be studied (notice that a very deep network and a same readout operation for each node [\textcolor{blue}2] are not global).
% We believe the discussion on locality, as said by reviewer 1, can help designing global AC-GNNs for similar tasks.
% and only global algorithms can be optimal in the MIS problem.
Below is our response to the major concerns:
% Code will be made public to ensure reproducibility. We address each individual concern as follows.
% We would like to emphasize that one of the most important novelties of our paper 
% is the theoretical study about the relationship between an $r$-local algorithm and global algorithm.
% Given a 
% \section{}
\\[5pt]
\noindent \textbf{\large To Reviewer1}  
% We first appreciate the detailed feedback by reviewer 1, especially finding a seriously ambiguous statement in P3: 
% we should analyze the ability to assign \textit{connected} nodes different colors. 
% (although the discussion in the context helps readers to understand correctly.)
% Actually, reviewer 1 has a deep understanding on our paper. 
% However, 
\textbf{Summary of our first half}.
We start our discussion by the fact that a powerful GNN in coloring should assign {connected} nodes different colors. 
Based on this requirement under heterophily, the benefit of random node initialization is only one of our conclusions.
The discussion of the locality, injective function, and the drawback of integrated AC-GNN
are also derived from the requirement under heterophily.
Therefore, rather than several independent trivial observations, our analysis is more like several branches stem from the heterophily requirement and with theoretical proof.
\textbf{Trivial and already known observations (contributions)}.
Rather than a standard GNN architecture for general purpose, 
our work is specifically for coloring, a representative task under heterophily.
Although some rules are discussed in previous work like the benefit of randomness in GNN,
whether these rules are correct in heterophily is still an open question.
For example, in previous study under homophily, 
deeper GNNs often suffer from over-smooth problem (Zhao and Akoglu 2019) and it is believed that deepening GNNs do not improve (or sometimes worsen) their performance (Oono and Suzuki 2019).
Another case is about the advantage of injective function, it is also proved to enhance the power of GNNs under homophily (Xu et al. 2018),
and we prove it is still beneficial under heterophily.
Therefore, even though some related conclusions were derived, 
it was difficult for us to determine whether those conclusions still held (injective) or not (deep) in the coloring case.
Hence, one of our contributions is to give simple but effective guidance about the GNN architecture for the coloring problem.
Moreover, these guidance can be extended to tasks under heterophily.
\textbf{Network and training setting.}
These settings are covered in P8 of appendix. Other un-covered settings are stored in color\_arg.py as mentioned in the appendix. 
\textbf{Fig 2}.
Except for the model structure, all AC-GNN variations keep the same parameters and settings, such as the same random initialization, and the same preprocess and post-process.
We mention that they use the same training parameters in the appendix,
% but it can be inferred that fig 2 uses a random initialization since the results of all-one vectors are already shown in Tab 1.
% This is also 
\textbf{Tab 2}.
The training time is about 1 hour, which is mentioned in appendix. 
Therefore, even adding up the training time, our method is still much faster than tabucol in large graphs.
\textbf{Compared methods.}
In terms of non-neural methods, we compare the classic tabucol in the manuscript;
% In the manuscript, we consider AC-GNN variations, another NN-based coloring work, .
We also compare ILP (an optimal method) and the greedy heuristic explained before and its variations (static;dynamic;sorted) in the appendix.
% \textbf{}
% We follow the mathematical format in \cite{xu2018powerful,loukas2019graph}, which use $\{\}$ to represent a multi-set.
\textbf{Tab 1}
It uses the layout dataset (mentioned in the manuscript). The only difference with the default training setting in Fig 2 is the all-ones node attributes.
\textbf{Proof in P4}
The question to be proved is a paraphrase of Corollary 1, whose proof is given in the appendix.
We will change the order of the two paragraphs to avoid misunderstanding.
\textbf{global}
We formally defined what a local method is (def 2). 
A global method is the one that is not local. 
\textbf{$r$-local topologically equivalent} 
The node pair $\{u,v\}$ is \textit{$r$-local topologically equivalent}
if $\pi_r$ is an isomorphism from $\gB_{\gG}(u,r)$ to $\gB_{\gG}(v,r)$.
\textbf{$\vx-k$ \&``connected nodes" \& Multi-set}
Thanks for pointing out them.
We will update them in the revised version.
\\[5pt]
\noindent \textbf{\large To Reviewer2} 

\textbf{Compared methods.}
We use the latest optimized version of the open-source hybridEA as our another baseline.
Due to time limit, we only show the results of COLOR dataset here.
We follow the same setting in the paper:
population size = 10; $L$ = 2000; $A$ = 10; $\alpha$ = 0.6;
% The maximum number of iteration is 10$n$, where $n$ is the number of nodes.
Part of the results are shown in the table above, the first row is the cost and the second row is the time in milliseconds.
The first three columns are the results of Queen8\_12 (11\_11,13\_13) and the last column is the ratio with our method.
\begin{table}[]
    \begin{tabular}{llll} 
        % \toprule
  3     & 22     & 37     & 0.77 \\ \hline
 92947 & 141338 & 213026 & 395.63 \\
%  \bottomrule
    \end{tabular}
    \end{table}
Besides tabucol and hybridEA, we also compare it with an optimal method, ILP, in the appendix.
% We only compare it using the relatively small layout dataset, otherwise ILP fails to color the graph within an acceptable time.
According to the results, \textit{our method achieves exactly the same performance as ILP, which means ours is also optimal, in most layout graphs}.
\textbf{Preprocess.}
When we dismiss the preprocess, the cost of our method is increased by 5.3\% and the runtime is reduced by 2.8\%.
the runtime of ILP and tabucol without preprocess explodes in some graphs and fail to get the results within three hours.
We did not discuss the results without preprocess in the manuscript because the preprocess was applied for all methods, and made our method advantageous and even unfair to compare with other methods 
(both ILP and tabucol are not good at large sparse graphs and must require pre-process).
\\[5pt]
\noindent \textbf{\large To Reviewer3} 
\textbf{Further impact and applications.}
Most of our analyses are based on the requirement under heterophily: 
a powerful GNN under heterophily should assign {connected} nodes as different features as possible.
Therefore, our proved rules (except the color-equivariant one) can be directly applied in other tasks under heterophily such as MIS, SAT.
\\[5pt]
\noindent \textbf{\large To Reviewer4} 
\textbf{Motivations.}
We are sorry that our motivation is not clearly stated.
We try to study the performance of GNNs for the coloring problem because
1) Graph coloring and its variations have a great demand in industry. 
Moreover, the target graph size becomes too large to be processed by general heuristic algorithms within an acceptable time.
For example, the netlist graph in a commercial chip contains millions of gate nodes;
the size of the user graph in Internet company is also at a million level.
Therefore, these requirements from GNNs motivate us to apply the power of highly parallelable GNNs.
2) 
Graph coloring problem is the most classical one under heterophily.
On the other hand,
as we mentioned, ``most of existing GNNs even cannot beat the simplest heuristic algorithm".
Therefore, in this paper, we try to find the reason for the low performance
so that we can provide some theoretical guidance on a powerful GNN for all tasks under heterophily.
\textbf{color equivarience.}
Thanks for pointing out it.
We will update them in the revised version.
\textbf{rules results.}
The ablation study of rules (except rule 5) is given in the ablation study sec. of appendix.
Rule 5 studies the color equivariance property of GNNs, therefore,
it does not influence the solved ratio but only the fixed color ratio, where the result is given in Fig 2b.


==> doc/related.tex <==
\section{Related works}
\label{sec:related}
\paragraph{Local vs. global.}

% Our definition of \textit{a maximally powerful GNN} is a direct rephrasing of L5, P2, [\textcolor{blue}7].
% Your definition differs with ours only because we discuss ``maximal power'' from different perspectives.
% From the perspective of AC-GNNs, the depth (\# of layers) of any AC-GNN is always finite, say $r$,
% then, a maximally powerful AC-GNN with depth $r$ can be identified by r-local equivalence. 
% From the perspective of graph, as you \textcolor{black}{mentioned}, it should be identified by the ``global'' equivalence, i.e., covering the full graph.

The reception fields of GNNs haven been shown to be limited by its depth \cite{xu2018powerful,barcelo2019logical,morris2019weisfeiler}.
To tackle with the locality limitations and make GNNs able to detect the global graph structure, considerable attention has been paid to either introduce operation containing global information \cite{barcelo2019logical,li2020distance,you2019position,pei2020geom,rong2019dropedge}
or increase the model depth \cite{xu2018representation}.
Nevertheless, some variations of AC-GNN are still local \textit{for the graph coloring problem} if the global features applied also fail to discriminate the local equivalent node pairs according to definition \ref{def:local}.
For example, \cite{barcelo2019logical} uses a readout operation that assigns each node a global feature calculated by the summation of all node features.
The summation feature, however, keeps the same for all nodes and thus fails to help discriminate the local equivalent node pair.
On the contrary, some methods succeed in distinguishing the local equivalent node pair without a global mechanism such as DropEdge \cite{rong2019dropedge}, which drops edge randomly in each layer and thus breaks the local equality.

\paragraph{Graph coloring algorithms.}

A good node embedding procedure should be injective, but also smooth. Therefore, mapping nodes surrounded by similar topologies to similar feature vectors.


\paragraph{GNNs for NP-hard problems.}
